FrameQuant: Flexible Low-Bit Quantization for Transformers

Transformers are the backbone of powerful foundation models for many Vision and Natural Language Processing tasks. But their compute and memory/storage footprint is large, and so, serving such models is expensive often requiring high-end hardware. To mitigate this difficulty, Post-Training Quantization seeks to modify a pre-trained model and quantize it to eight bits or lower, significantly boosting compute/memory/latency efficiency. Such models have been successfully quantized to four bits with some performance loss. In this work, we outline a simple scheme to quantize Transformer-based models to just two bits (plus some overhead) with only a small drop in accuracy. Key to our formulation is a concept borrowed from Harmonic analysis called Fusion Frames. Our main finding is that the quantization must take place not in the original weight space, but instead in the Fusion Frame representations. If quantization is interpreted as the addition of noise, our casting of the problem allows invoking an extensive body of known consistent recovery and noise robustness guarantees. Further, if desired, de-noising filters are known in closed form. We show empirically, via a variety of experiments, that (almost) two-bit quantization for Transformer models promises sizable efficiency gains. The code is available at https://github.com/vsingh-group/FrameQuant

==> sec/inference_comp.tex <==
\comment{
\textcolor{red}{
\section{Storage and Inference Computational Complexity}
\begin{inparaenum}
\item {\em Storage:} Consider an example where we are quantizing a weight matrix $\Theta_l$ of dimension $1024 \times 1024$ using FrameQuant with a redundancy factor of $r = 1.1 \times$. The size of the original matrix using FP32 is 4MB. After transforming the weights to map within the FF representation space, the transformed weights $D_l$ have dimensions $1126 \times 1126$, which are quantized and represented using 2 bits. This quantized weight $\hat{D}_l$ has a size of 0.3MB. Along with the quantized weights, we need to store the bias and scale values for each row leading to an additional storage of 1024 FP32 values, which will incur an additional cost of 0.007MB. All this sums up to a storage of 0.307MB from an initial 4MB. Since we can generate the Fusion Frames on the fly, we just need to store the $(k, \rho, d)$ values, and a seed to generate the random rotation matrix which incurs negligible storage costs. \\
\item {\em Computations during Inference:} Since the Tight Fusion Frames generated by the algorithm described in section \ref{sec:tff_construction} has a block diagonal structure, transforming the quantized weights $\hat{D}_l$ from FF representation space to the regular weight space can be done efficiently in $\mathcal{O}(kd^2r)$. This can be small at low redundancy values and a small number of subspaces. Since we are also rotating the Fusion Frames, we need an additional computational computation of $\mathcal{O}(d^2 \sqrt{d})$ or $\mathcal{O}(d^2 \log (d))$ based on the choice of implementation of random orthogonal matrices. Note that any quantization scheme in the low-bit regime will incur a cost of $\mathcal{O}(d^2)$ to transform the quantized weights by scaling and shifting them. The sparse properties of the TFF construction and the efficient choice of random rotations make FrameQuant a great choice to trade off computational complexity and storage benefits while providing additional flexibility in terms of fractional bit widths. The details of these computations are in the Appendix \ref{Computational complexity calculation}.
\end{inparaenum}
}
}

==> sec/related_work.tex <==
\section{Related Work}
\label{sec:related work}
Where, $W$ are the true or unquantized weights, $\hat{W}$ are the quantized weights. $X$ is samples at random from the dataset. Previous work \cite{UpOrDown} have shown that this loss can be approximated using the quadratic term in the taylor expansion based on the Hessian $H$. Later, the work of \cite{OBQ}, \cite(GPTQ} developed an iterative algorithm based on this quadratic approximation, which applies the classical OBS framework to the task of pruning and quantization of Neural networks in an efficient manner. The main idea of these works is that they quantize a few parameters in a matrix at a time while adjusting the remaining weights that are not yet compressed to adjust for the change in loss due to the quantization of the current set of weights.

